Why Charles Can Pen-test: an Evolutionary Approach to Vulnerability Testing

Discovering vulnerabilities in applications of real-world complexity is a daunting task: a vulnerability may affect a single line of code, and yet it compromises the security of the entire application. Even worse, vulnerabilities may manifest only in exceptional circumstances that do not occur in the normal operation of the application. It is widely recognized that state-of-the-art penetration testing tools play a crucial role, and are routinely used, to dig up vulnerabilities. Yet penetration testing is still primarily a human-driven activity, and its effectiveness still depends on the skills and ingenuity of the security analyst driving the tool. In this paper, we propose a technique for the automatic discovery of vulnerabilities in event-based systems, such as web and mobile applications. Our approach is based on a collaborative, co-evolutionary and contract-driven search strategy that iteratively (i) executes a pool of test cases, (ii) identifies the most promising ones, and (iii) generates new test cases from them. The approach makes a synergistic combination of evolutionary algorithms where several "species" contribute to solving the problem: one species, the test species, evolves to find the target test case, i.e., the set of instruction whose execution lead to the vulnerable statement, whereas the other species, called contract species, evolve to select the parameters for the procedure calls needed to trigger the vulnerability. To assess the effectiveness of our approach, we implemented a working prototype and ran it against both a case study and a benchmark web application. The experimental results confirm that our tool automatically discovers and executes a number of injection flaw attacks that are out of reach for state-of-the-art web scanners.

==> app-log.tex <==
Oct 21, 2017 1:30:39 PM it.unige.cseclab.log.Log log 
INFO: Found API: <edu.ksu.cs.rawquery.LoginActivity: void onCreate(android.os.Bundle)>, ['148688130', ''], distance: 2.0
Oct 21, 2017 1:30:39 PM it.unige.cseclab.log.Log log 
INFO: Found API: <edu.ksu.cs.rawquery.MyContentProvider: android.database.Cursor query(android.net.Uri,java.lang.String[],java.lang.String,java.lang.String[],java.lang.String)>, ['160160909', '1048862490', , 'username = '' AND password = ''', , ''], distance: 1.0
Oct 21, 2017 1:30:39 PM it.unige.cseclab.log.Log log 
INFO: iter      fit     chromosome
Oct 21, 2017 1:30:39 PM it.unige.cseclab.log.Log log 
INFO: 0 27.0    [p3 := !0!' OR '1'='1';]
Oct 21, 2017 1:30:40 PM it.unige.cseclab.log.Log log 
INFO: 1 27.0    [p3 := !0!' OR '1'='1';]
Oct 21, 2017 1:30:40 PM it.unige.cseclab.log.Log log 
INFO: 2 27.0    [p3 := !0!' OR '1'='1';]
Oct 21, 2017 1:30:40 PM it.unige.cseclab.log.Log log 
INFO: 3 27.0    [p3 := !0!' OR '1'='1';]
Oct 21, 2017 1:30:40 PM it.unige.cseclab.log.Log log 
INFO: 4 27.0    [p3 := !0!' OR '1'='1';]
Oct 21, 2017 1:30:40 PM it.unige.cseclab.log.Log log 
INFO: Score: 0.9642857142857143

INFO: Found API: <edu.ksu.cs.rawquery.MyContentProvider: android.database.Cursor query(android.net.Uri,java.lang.String[],java.lang.String,java.lang.String[],java.lang.String)>, ['160160909', '104886249    0', , 'username = 'nameusernameusername' AND password = 'password@123$password@123$'p'', , '']
INFO: Score: 0.9864864864864865

Best Fitness: 0.9642857142857143
Test Actions: touch 812 241 >> type password@123$^@^@^@ >> touch 1050 430 >> touch 1070 382 >> type A    Q6N^@^@^@^@^@^@^@^@^@^@^@^@ >> touch 676 240 >> type 3G^@^@^@^@^@^@^@^@^@^@^@^@^@^@ >> type ='^@^@^@^    @^@^@^@^@^@^@^@^@^@^@ >> touch 1037 628 >> touch 607 708 >> touch 1069 519 >> touch 619 184 >> touch     613 686 >> touch 847 100 >> touch 786 221 >> type password@123$^@^@^@ >> touch 553 381 >> wait 0.3321    895 >> touch 833 699 >> type password@123$^@^@^@ >> touch 1060 376 >> type qLFz3^@^@^@^@^@^@^@^@^@^@^    @ >> touch 935 251 >> wait 0.35822493 >> touch 814 741 >> touch 694 825 >> touch 726 147 >> wait 0.73    34589 >> type xB@O0^@^@^@^@^@^@^@^@^@^@^@ >> touch 962 720 >>




==> approach.tex <==
\section{Approach}
\label{beagle:sec:approach}

\paragraph*{Vulnerabilities} are stored in a digested format, using the required call trace for their activation.
\paragraph*{Call Precondition Inference} infers the Call Preconditions based on the desired vulnerability. Call Preconditions are inferred with Hoare Logic.
\paragraph*{Call Graph Generator} takes an APK and a Call Precondition as input. It generates an Call Graph of the code contained in the APK and annotates each call with the distance from the desired Call.
\paragraph*{APK Inliner} takes an APK and a Call Precondition as input. It generates an Instrumented APK by modifying the code of the original application in order to log target method calls and their parameters. This APK is installed on a device (real or emulated).
\paragraph*{Genetic Engine} generates a set of \textit{chromosomes} consisting in possible sequences user actions. Chromosomes are translated in \textbf{test cases} and later passed to a \textbf{Test Execution Engine} that implements them on a device.
The device running the Instrumented APK produces a \textbf{System Log} containing monitored method calls. This log is sent back to the Genetic Engine, which calculates current \textbf{fitness} values and evolves the chromosome set.


==> preamble.tex <==
% Names
\newcommand{\toolname}[1]{Beagle}
\newcommand{\casestudyapp}[1]{{\sc scw}}

%%%% Comandi per icone cromosomi
\newcommand{\drag}[1]{\faArrows}
\newcommand{\click}[1]{\faHandPointerO}
\newcommand{\wait}[1]{\faClockO}
\newcommand{\type}[1]{\faKeyboardO}


\newcommand{\orsyn}{\ensuremath{\:\mid\:}}
\newcommand{\qed}{\hfill\ensuremath{\blacksquare}}

\newcounter{example}
\newenvironment{example}[1][]{\refstepcounter{example}\noindent
   \textbf{Example~\theexample. #1} \rmfamily}{\qed}

\newcounter{definition}
\newenvironment{definition}[1][]{\refstepcounter{definition}\noindent
   \textbf{Definition~\thedefinition. #1}}{\qed}

\pgfplotsset{%
    ,compat=1.12
    ,every axis x label/.style={at={(current axis.right of origin)},anchor=north west}
    ,every axis y label/.style={at={(current axis.above origin)},anchor=north east}
    }

\VerbatimFootnotes


==> vulnerability.tex <==
\section{Vulnerability specification}
\label{beagle:sec:vulnerability}

%A vulnerability is a pair $\langle P, S \rangle$ where $P$ is a predicate and $S$ is a method signature.
%A \emph{signature} is the unique identifier of a method.
%Its format is 
%\vspace{-2pt}
%$$Cls : \tau_r \: Meth(\tau_1\; Var_1, \ldots, \tau_n\; Var_n)$$ 
%\noindent
%where $Cls$ is the class declaring the method, $\tau_r$ is its return type, i.e., a basic type, a class or void, $Meth$ is the name of the method and $Var_i$ it its $i$th parameter of type $\tau_i$.
%Predicates are expressed through the abstract syntax of Table~\ref{tab:vulnsyntax}.
%
%\begin{table}[t]
%\begin{tabular}{l @{\hspace{8pt}} l}
%\begin{tabular}{l @{\,::=\:} l}
%$P$ & $A_P \orsyn \neg P \orsyn P \vee P  \orsyn P \wedge P$ \\
%$A_P$ & $B_A$ \orsyn $B_O$ \orsyn $B_S$ \orsyn $B_B$ \\
%$B_A$ & $A_E > A_E$ \orsyn $A_E < A_E$ \orsyn $A_E = A_E$\\
%$A_E$ & $A_V$ \orsyn $A_E \oplus A_E$ \orsyn \verb|len|$(Str)$  \\
%$A_V$ & $Num$ \orsyn $Var$ \\
%\end{tabular} &
%\begin{tabular}{l @{\,::=\:} l}
%$B_O$ & $O_V$ \verb|equals| $O_V$ \\ % \!\!\orsyn $O_V$ \verb|typeof| $Cls$
%$O_V$ & \verb|null| \orsyn $Var$ \\
%$B_S$ & $Var \in R_E$ \\
%$R_E$ & $Str \!\orsyn \!R_E \!\cdot\! R_E\! \orsyn R_E\! +\! R_E \orsyn\! R_E^\ast$ \\
%$B_B$ & $\mathtt{true}$ \orsyn $\mathtt{false}$ \orsyn $Var$
%\end{tabular}
%\end{tabular}
%\caption{The vulnerability specification syntax.}
%\label{tab:vulnsyntax}
%\end{table}
%
%%\avnote{la grammatica delle regex esce dal bordo - DONE}
%A predicate $P$ is either an atomic predicate $A_P$ or a composition of sub-predicates through the standard logic operators.
%An atomic predicate is an expression over the integers ($B_A$), objects ($B_O$), strings ($B_S$) or boolean values ($B_B$).
%Comparisons between arithmetic expressions $A_E$ are standard and we feel free to introduce some syntactic sugar, e.g. $x \leq y$ for $x < y \,\vee\, x = y$.
%Also arithmetic expressions $A_E$ are standard (for brevity we denote them with $A_E \oplus A_E$).
%Only note that an arithmetic expression can also be the length of a string $s$, i.e., \verb|len|$(s)$.
%An atomic expression $A_V$ is either a number $n \in Num$ or a variable $x \in Var$.
%An object ($O_V$), which is either \verb|null| or a variable, can be compared ($B_O$) with another one (\verb|equals|).
%String expressions ($B_S$) reduce to checking whether a string variable belongs to the language generated by a regular expression $R_E$.
%Regular expressions are standard and we assume the reader to be familiar with them.
%Finally, boolean atoms ($B_B$) are either constants or variables.
%
%\begin{example}
%\label{ex:specvuln}
%Consider the following vulnerability specification (inspired by~\cite{Kiezun09hampi}).
%\[
%\left\langle
%\begin{array}{c}
%\verb|args equals null| \wedge \verb|q| \in R_{SQL} \cdot \verb|" OR 1=1"| \\
%\verb|SQLiteDatabase : Cursor rawQuery(String q, String[] args)|
%\end{array}
%\right\rangle
%\]
%It defines an abstract exploitation of a SQL injection vulnerability over the \texttt{rawQuery} method.
%The vulnerability is enabled when an attacker can append a disjunction with a tautological statement, i.e., \verb|OR 1=1|, at the end of a SQL query $R_{SQL}$ which is an abbreviation for 
%
%\noindent
%\begin{center}
%$R_{SQL} = \verb|"SELECT "| \cdot \Sigma^+ \cdot \verb|" FROM "| \cdot \Sigma^+ \cdot \verb|" WHERE "| \cdot \Sigma^+$
%\end{center}
%
%\noindent
%where $\Sigma$ stands for any character and $\Sigma^+$ is an abbreviation for $\Sigma \cdot \Sigma^\ast$.
%\end{example}


==> weakest.tex <==
\section{Weakest preconditions}
\label{beagle:sec:weakest}

